Axiomatic Ranking of Network Role Similarity

A key task in social network and other complex network analysis is role analysis: describing and categorizing nodes according to how they interact with other nodes. Two nodes have the same role if they interact with equivalent sets of neighbors. The most fundamental role equivalence is automorphic equivalence. Unfortunately, the fastest algorithms known for graph automorphism are nonpolynomial. Moreover, since exact equivalence may be rare, a more meaningful task is to measure the role similarity between any two nodes. This task is closely related to the structural or link-based similarity problem that SimRank attempts to solve. However, SimRank and most of its offshoots are not sufficient because they do not fully recognize automorphically or structurally equivalent nodes. In this paper we tackle two problems. First, what are the necessary properties for a role similarity measure or metric? Second, how can we derive a role similarity measure satisfying these properties? For the first problem, we justify several axiomatic properties necessary for a role similarity measure or metric: range, maximal similarity, automorphic equivalence, transitive similarity, and the triangle inequality. For the second problem, we present RoleSim, a new similarity metric with a simple iterative computational method. We rigorously prove that RoleSim satisfies all the axiomatic properties. We also introduce an iceberg RoleSim algorithm which can guarantee to discover all pairs with RoleSim score no less than a user-defined threshold $\theta$ without computing the RoleSim for every pair. We demonstrate the superior interpretative power of RoleSim on both both synthetic and real datasets.

==> Problem.tex <==

\section{Background}
\label{section:problem}

In this section, we develop a precise yet general definition of structural role in a network that has a natural social interpretation and is easily represented in mathematical terms.  Our definition is quite general; it encompasses existing definitions as special cases and suggestions alternative specific realizations.  We begin by looking at past approaches to identifying roles in a network.

Social network analysis is a subfield of sociology where graph theory, matrix algebra, and other mathematical methods are used to study networks of social relationships.  According to some practitioners[], a {\em role} is the set of interactions of an actor (vertex), whereas a {\em position} is the set of all actors (vertices) who have the same or similar roles. However, even some social scientists use these, terms interchangeable, so we will simply use role, where its meaning should be clear from the context.

\subsection{Equivalence Classes}
In social network analysis, the traditional approach to formalizing the defintion of role and role group is to define a equivalence class. Actors who fulfill the same role are equivalent. Over the years, three definitions, offering different degrees of strictness, have stood out.  These three, in chronological and decreasing strictness order, are structural equivalence, automorphic equivalence, and regular equivalence. Two actors are {\bf structurally equivalent} if they interact with exactly the same set of others.  That is, if $a$ interacts only with $c$ and $d$, then for $b$ to be structurally equivalent to $a$, it must also interact only with $c$ and $d$.  This definition is too limiting for most applications.

Two actors are {\bf automorphically equivalent} if there is a mapping of the original graph to an isomorphic graph which maps the first actor to the second one.  From a more intuitive or social perspective, if we ignore names and consider the topology, then the first actor's relationships look the same as the second's. In fact, since we require an isomorphism for the entire graph, the equivalance holds not just for an actor's direct neighbors, but also for its indrect neighbors, e.g., friends of friends. For example, consider a graph consisting of two families that each have a mother, father, two sons, and one daughter.  The two mothers are sisters to one another. The two mothers are automorphically equivalent.  Note that a full description of their direct roles would be "sister, wife, mother of two sons, and mother of one daughter."  Indirect roles include sister-in-law and aunt. Structural equivalance is a special case of automorphic equivalence.

Two actors are {\bf regularly equivalent} if they interact with the same class of others, where class is recurively defined by regular equivalence.  The effect of looking at interactions based on class rather than individual identity has two effects.  First, cardinality within a class does not matter.  For example, in our previous family network, if one family has an additional child, the two mothers would no longer be automorphically equivalent, but they would still be regularly equivalent. Second, since class is defined recursively, the idea of neighborhood extends to infinite distance.  Automorphic equivalence is a special case of regular equivalence.

\comment{
Most of the recent practical work has used regular equivalence, because the cardinality relaxation seems to be necessary, and algorithmic tools have been developed for researchers to use [REGE, CATREGE].  However, our contention is that cardinality does matter, but it should be a weighting factor, not an accept/reject rule.  Let us develop a clearer definition of role:
} % end comment

\subsection{Role Assignment as Coloring}
Each of these equivalences can be described in terms of what a vertex sees when it observes its neighbors.
Assigning a vertex to a class is the same as vertex labeling or generalized vertex coloring.  Unlike standard vertex coloring, our constraint is not that adjacent vertices cannot be the same color.  Instead, our objective is to find a coloring such that two vertices of the same color each see the same or similiar spectra (distributions of colors) when they observe their own neighborhoods.

We will use the following terminology in this paper.  $G = (V, E)$ is a directed graph with vertex set $V = \{v_1,...,v_n\}$. $R = \{r_1,...,r_k\}$ is a set of colors.  Let every vertex $v \in V$ have a color label $r(v), r(v) \in R$.  Let $I^v = \{i^v_1, i^v_2,...,i^v_n\}$ be the set of in-neighbors of $v$ and $O^v = \{o^v_1, o^v_2,...,o^v_m\}$ be its out-neighbors.

\bdefin {\bf Neighbor color spectra.}
The in-neighbor spectrum, or {\em I-spectrum} of $v$ is the vector $F^v_i = (f(I^v,c_1),...,f(I^v,c_s))$, where $f(u)$ is a non-negative increasing function of either 
.  Similarly, the out-neighbor spectrum  or {\em O-spectrum} is $F^v_o = (f(O^v,c_1),...,f(O^v,c_k))$.  $F^v_i(j)$ refers to $j^th$ element of the vector, the spectral component for color $c_j$.
\edefin

We now provide a general description of the Role Coloring Problem:\\

\bdefin {\bf Role coloring problem.}
Let $G = (V,E)$ be a directed graph.  The role coloring problem is to assign each vertex $v$ a role $c(v)$ such that for any two vertices $u$ and $v$ where $c(u) = c(v)$,\\
(1) their I-spectra $C(I_u)$ and $C(I_v)$ are similar, and \\
(2) their O-spectra $C(O_u)$ and $C(O_v)$ are similar.
\edefin

This general model encompasses structural equivalence, automorphic equivalence, and regular equivalence, depending on how the spectra are defined.  For structural equivalence, the individual identity of each neighbor is important, not its role.  Therefore, every vertex should be assigned a different color, implying that $k = |V|$.  For automorphic equivalence, we want to match exact numbers of roles.  Thus, $f$ counts how many times each color appears in the neighborhood.  For regular equivalence, we only care about role types but not quantity.  In this case, $f(j) = 1$ if the neighborhood contains at least one neighbor with color $c_j$; otherwise $f(j) = 0$.  Table \ref{spectra} summarizes the spectral functions used for the different equivalence models.

\begin{table}[h]
\centering
\small
\begin{tabular}{|c|p{0.75in}|c|} \hline
Equivalence & Spectrum vector length & Value of $i^{th}$ element \\ \hline
Structural  & |V| (vertices) & 1 if $v_i \in N^v$; else 0 \\ \hline
Automorphic & k (colors)  & $|\{u \in N^v, r(u) = r_i\}|$ \\ \hline
Regular     & k (colors)   & 1 if $\exists u \in N^v, r(u) = r_i$; else 0 \\ \hline
\end{tabular}
\caption{Spectral Vectors for Equivalence Classes} \label{spectra}
\end{table}


{\bf Optimal Role Coloring Problem}\\
Let $G = (V,E)$ be a directed graph.  Assign each vertex $v$ a role $c(v)$ such that for any two vertices $u$ and $v$ where $c(u) = c(v)$,\\
(1) their I-spectra $C(I_u)$ and $C(I_v)$ are similar, and \\
(2) their O-spectra $C(O_u)$ and $C(O_v)$ are similar,\\
(3) the number of roles is minimized,\\
(4) the mutual similarity with each color set $\kappa(c_i) = \{v ] in V, c(v) = c_i\}$ is minimized.

Regular equivalence is the loosest definition, and many researchers have concluded that regular equivalence is the most practical metric for real-world networks.  This is reasonable, if one intended to seek only perfect equivalences.  However, if one is interesting in approximate matches, which is usually the case in the real-world, then automorphic equivalence is the best metric.  It perceived both the self and neighbors in terms of their roles, which structural equivalence does not.  It also maintains focuses on the cardinality of connections, which regular equivalence does not.  While not always the case, in many applications the number of connections is vitally importance.  In marketing, a person's influence is directly related to the number of important actors that can be reached, in a small number of steps.  In phone service, customers who call to or receive from many other persobs might be interested in certain services, such as speed dialing, volume discounts, and voice mail, while low-volume customers would have different interests. In this paper, we will develop models and solutions for automorphic equivalence, with regular equivalence being a degenerate case.  

Referring to this definition, it is easy to see how role discovery differs from other kinds of network pattern analysis.  In component discovery[], one seeks subgraphs whose vertices are highly interconnected; however, density of connections is not a consideration for roles.  In role analysis, we want to understand all the different groups that a role tends to connect to; internal connections are no more or less important than other group-group connections. In frequent subgraph pattern mining[], we look for isomorphically equivalent subgraphs that occur frequently.  For this problem, any subgraph may be considered, but for role analysis, we must look at a vertice's entire neighborhood.  We cannot focus on only a subset of neighbors, as pattern mining does. More importantly, in frequent pattern mining, vertices can be unlabeled, and a pattern can be fully described independent of its position in the graph.  On the contrary, a role is a label, whose value depends on a vertex's position within the content of the entire graph.



\comment{
Probably cut this:\\
We point out that there is no unique regular equivalence role assignment for a graph, because regular equivalence does not demand parsimony.  Consider the clique of a complete graph. Due to symmetry, we could say that every vertex is equivalent, so there is only one role.  Conversely, we could color every vertex differently and say that there are $n$ different roles with one member each. Consequently, the idea of an optimal assignment hinges on finding the smallest number of roles such that each actor's actual role is sufficient similar to others in its cohort.

Several algorithms have been produced to measure similarity of vertices.  However, none of these follow the exact needs of role similarly.  For example, several authors have noted the similarity between the SimRank metric [] and the definition of regular equivalence and declared them to be the same or sufficiently so.  In SimRank, the similarity between two vertices $u$ and $v$ is defined as
The similarity between vertices $u$ and $v$ is
\[ S(u,v) = \frac{1}{|N(u)||N(v)|} \sum_{x \in N(u)} \sum_{y \in N(v)} S(x,y) \]
with the overriding rule that $(v,v) = 1$.  However, SimRank diverges from true role similarity in several respects: weighting, path length, and initialization.  We provide further detail and improvements in the next section.

[Leicht] uses the relation $S_{ij} = \phi \sum_v A_{iv}S_{vj} + \psi \delta_{ij}$.  That is, they say $i$ is similar to $j$ if $i$'s neighbors are similar to $j$.  This definition inserts a one-sided direct adjacency into the computation, whereas there should be none according our understanding of role.

Rather than offering yet another similarity metric, we offer an ensemble of clustering methods to produce a consensus role grouping.  
}

\subsection{Block Model for Roles}







